Long Short-Term Preference Modeling for Continuous-Time Sequential Recommendation

Modeling the evolution of user preference is essential in recommender systems. Recently, dynamic graph-based methods have been studied and achieved SOTA for recommendation, majority of which focus on user's stable long-term preference. However, in real-world scenario, user's short-term preference evolves over time dynamically. Although there exists sequential methods that attempt to capture it, how to model the evolution of short-term preference with dynamic graph-based methods has not been well-addressed yet. In particular: 1) existing methods do not explicitly encode and capture the evolution of short-term preference as sequential methods do; 2) simply using last few interactions is not enough for modeling the changing trend. In this paper, we propose Long Short-Term Preference Modeling for Continuous-Time Sequential Recommendation (LSTSR) to capture the evolution of short-term preference under dynamic graph. Specifically, we explicitly encode short-term preference and optimize it via memory mechanism, which has three key operations: Message, Aggregate and Update. Our memory mechanism can not only store one-hop information, but also trigger with new interactions online. Extensive experiments conducted on five public datasets show that LSTSR consistently outperforms many state-of-the-art recommendation methods across various lines.

==> 03other/010intro.tex <==









With the rapidly expanding information on the Internet, recommender systems have become an integral part of online services for helping users alleviate the problem of information overload, such as enormous products, news, videos, and advertisements \cite{gao2021graph,wu2022graph}.
To recommend new items to a user, a traditional recommender system makes use of historical user-item interactions (e.g.\ clicking, purchasing) for collaborative signals \cite{wang2019neural,he2020lightgcn}, i.e., users who interacted with similar items are assumed to interact with the same item in the future. Unlike traditional recommender systems that model user preference in a static fashion, a sequential recommender system \cite{hidasi2016sessionbaseda,kang2018selfattentive} is capable of capturing user's evolving and dynamic preference. User preference can be arguably factorized to two parts, namely \textit{long-term} preference and \textit{short-term} preference. The long-term preference refers to inherent and relatively stable purchasing bias, e.g.\ favorite colors, preferred brands, and affordable price \cite{zhou2018deep,feng2019deep}. The short-term preference conveys user's interaction intention in a relatively short period, e.g.\ within days or even a session. 

To model the dynamics of user preference, existing work on sequential recommender system takes user-item interactions as a sequence rather than a set. By considering the order of interactions, sequential recommender systems capture the temporal dimension of high-order collaborative signals. Specifically, early efforts leverage Markov chain \cite{rendle2010factorizing}, CNN \cite{tang2018personalized}, or RNN \cite{hidasi2016sessionbaseda} to capture either short-term preference or long-term dependency. Some recent studies \cite{li2017neural,liu2018stamp,wu2019sessionbased} jointly model long short-term preference through global embedding and local embedding, respectively. Moreover, self-attention mechanism \cite{vaswani2017attention} is used to adaptively fuse information of recent interactions and overall preference \cite{kang2018selfattentive,li2020time,chang2021sequential}. However, this approach ignores the continuous nature of time, limiting the ability of sequential recommender system to capture fine-grained temporal signals. For example, given two users with the same sequence of interacted items, while one completes the interactions in one day and the other lasts for one month, the preference of the former user is considered to transit more rapidly. This information can potentially improves recommendation quality. Recent studies \cite{kumar2019predicting,li2020time,fan2021continuoustime} on the \textit{continuous-time sequential recommendation} problem, where recommendation is made for a specified time point, propose to encode time interval together with the sequence and show promising results.

Despite their effectiveness, two major challenges in sequential recommendation have not been well-addressed so far. (1) While continuous time and long short-term preference are two important characteristics of user-item interactions, it is unclear if the two can be jointly modeled. (2) Model complexity increases dramatically due to the consideration of continuous time. To address these two challenges, we approach the sequential recommendation problem with respect to both continuous time and long short-term preference. This joint approach is beneficial to accurately modeling both periodic and recent interactions. For example, a user would regularly have coffee for breakfast (long-term), but the choice for dinner may vary regarding recent interest (short-term). In this case, information of continuous time is required to distinguish between breakfast and dinner, and special care is also needed to model both long and short-term preferences.

Specifically, we present the Long Short-Term Preference Modeling for Continuous-Time Sequential Recommendation (\modelname), which takes user-item interactions associated with timestamp and features as input, and recommends items for a given user at a specified time point. Our method consists of three components. (1) Long Short-Term Preference Modeling module encodes long-term preference as global embedding, and updates short-term preference embedding by a memory mechanism. The memory mechanism is continuous time-aware so that the impact of recent interactions can be adaptively determined. (2) Dynamic Collaborative Filter Modeling module produces representation for users and items at a given time point, by combining the long short-term embedding and features. This module utilizes dynamic self-attention collaborative filter (DSACF), thus, the method can capture fine-grained dynamic collaborative signals. (3) The recommendation and optimization module takes user and item representation as input, and outputs a ranked list of items for a given user at a given timestamp.

Our experiments show that the \modelname method significantly outperforms various baseline methods over three datasets. Further analysis indicates the dynamic graph-based collaborative filtering module benefits from the long short-term embedding module, as the latter provides two different views (long and short) of past user interactions. Compared to other graph-based methods like TGSRec \cite{fan2021continuoustime}, the \modelname method requires fewer hops of message passing,
% message passing in the help of the embedding module, 
which in turn speeds up the training 5x and inference by 10x. The contributions of our work are summarized as 

\begin{itemize}[leftmargin=*]
\item We connect continuous-time sequential recommendation with long short-term preference modeling, which enables capturing dynamic collaborative signals from different views.
\item We propose the \modelname method, with respect to both continuous time and long short-term preference. % [fix] 此条contribution包含下一条
And we design a long short-term preference modeling, which explicitly encodes long short-term preference. This overcomes the problem that long short-term preference cannot be modeled effectively in continuous-time sequential recommendation. 
% Our method is able to use only one layer of graph attention speeds up the method dramatically owing to memory mechanism.
\item We conduct empirical experiments on three public datasets. Extensive results demonstrate the state-of-the-art performance of \modelname and its efficiency in the training and inference process.
\end{itemize}



